Following the Data, Not the Function: Rethinking Function Orchestration in Serverless Computing

Serverless applications are typically composed of function workflows in which multiple short-lived functions are triggered to exchange data in response to events or state changes. Current serverless platforms coordinate and trigger functions by following high-level invocation dependencies but are oblivious to the underlying data exchanges between functions. This design is neither efficient nor easy to use in orchestrating complex workflows -- developers often have to manage complex function interactions by themselves, with customized implementation and unsatisfactory performance. In this paper, we argue that function orchestration should follow a data-centric approach. In our design, the platform provides a data bucket abstraction to hold the intermediate data generated by functions. Developers can use a rich set of data trigger primitives to control when and how the output of each function should be passed to the next functions in a workflow. By making data consumption explicit and allowing it to trigger functions and drive the workflow, complex function interactions can be easily and efficiently supported. We present Pheromone -- a scalable, low-latency serverless platform following this data-centric design. Compared to well-established commercial and open-source platforms, Pheromone cuts the latencies of function interactions and data exchanges by orders of magnitude, scales to large workflows, and enables easy implementation of complex applications.

==> contents/background_outdated.tex <==
%!TEX root=../paper.tex
\section{Background and Motivation}
\label{sec:motivation}

In this section, we briefly describe the general serverless function orchestration model workflow DAG(\S\ref{sec:serverless_orchestration}), diverse needs of function interactions in serverless applications (\S\ref{sec:serverless_app}). 
Then, we illustrate the current approach to deploying applications and its common problems (\S\ref{sec:deploy_app}). At the end, we highlight the requirements for FaaS platforms (\S\ref{sec:faas_requirement}).
% , motivating the need for .
{\color{red}
\subsection{Serverless Function Orchestration}
\label{sec:serverless_orchestration}

Current FaaS platforms generally model an application as a workflow DAG~\cite{akkus_sand:_2018, knix,sreekanti_cloudburst_2020, kotni_faastlane_nodate, mahgoub_sonic_nodate, open_whisk_composer,google_cloud_composer,aws_step_function}, where the nodes represent functions and edges indicate the invocation and data flows among them.
The functions get triggered and transfer data with others following the order specified in the workflow.
The workflow DAG can be described via programming languages (e.g., Python)~\cite{open_whisk_composer,google_cloud_composer} or DSL (e.g., Amazon States Language)~\cite{knix, aws_step_function}. For example, in \cite{aws_step_function}, a typically workflow-based serverless platform, each function in the workflow is registered at first. Then, clients specify each function in the workflow and how they are composed to form a computation graph. Nodes in this graph either invoke a serverless function (or some other cloud service), forwarding its output to a specified target node, or they inspect their input
to make a conditional state transition.

To enable communication between serverless functions, workflow-based platform manage shared state in different manners, such as function composition, direct communication, and shared mutable storage. We want to stress in this section that these solutions are still insufficient when building nowadays serverless applications.
}

\subsection{Serverless Applications}
\label{sec:serverless_app}
Serverless cloud allows users to deploy their code as functions with the promise of seamless and automatic scaling.
Due to the elasticity, researchers and practitioners increasingly leverage serverless functions to boost many real-world applications, including web services~\cite{aws_lambda}, IoT applications~\cite{lambda_scenarios}, data analytics~\cite{jonas_occupy_2017,pu_shuffling_2019,zhang_caerus_nodate}, video processing~\cite{fouladi_encoding_nodate, ao_sprocket_2018}, and so on.
An application is backed by a set of interacting functions.
Since these applications can have radically different execution patterns and performance requirements, deploying them in the serverless cloud introduces diverse needs of function interactions.
% Due to the diverse needs of function interactions, deploying such a wide variety of applications would be a challenging task for developers, 
% especially in the settings that functions have no direct communications.
% Today's serverless applications vary greatly in the patterns they triggers functions share data among them.
For example, latency-sensitive applications like microservices cannot tolerate high delays of function invocations and message passing, sometimes only allowing microsecond-scale overheads~\cite{jia_nightcore_2021,boucher_putting_2018}.
Analytical workloads can need a large number of parallel functions that exchange and process a considerable amount of intermediate data~\cite{klimovic_pocket:_2018, pu_shuffling_2019}.
Streaming tasks are typically required to perform aggregation on accumulated data and deliver high throughput~\cite{xu_move_2021,chintapalli_benchmarking_2016}.

Many requirements for function interactions are difficult, or even infeasible, to fulfill by cloud users. Hence, there is a pressing need for FaaS platforms to allow developers easily and efficiently running a broad range of serverless applications.
We next summarize the requirements for a desired serverless platform.


\subsection{Deploying Applications Today}
\label{sec:deploy_app}

It is difficult to build and deploy many applications on current FaaS offerings.
We next discuss their limitations on expressiveness, usability and applicability.

% While this approach simplifies modeling the dependencies among functions, it could in practice impose constraints on developers due to three problems, which we discuss as follows.

\PHM{Expressiveness}


While workflow-based orchestration simplifies modeling the dependencies among functions, it disables flexible data sharing.
Running a serverless application typically requires the knowledge of function interactions in two aspects: (1) how functions are invoked, and (2) how they share intermediate data.
However, current workflow DAG only allows developers to specify the first, while there is almost no support for describing the patterns of data sharing, significantly limiting its expressiveness.
In particular, the DAG treats function call and data transfer as a whole, where a function passes its result to others by directly invoking them.
It hence requires functions having the same flows of invocations and data, which in fact does not hold in many applications, mandating developers to explore serverless solutions on their own.

We illustrate this via the examples in Fig.~\ref{fig:data_flow_example}.
When a analytical job performs the shuffle operation, it needs all-to-all data exchange among functions of two stages (Fig.~\ref{fig:data_flow_example} right).
Once the first stage completed, the workflow can invoke parallel functions in the second stage, but fail to directly transfer the data each function needs.
It forces developers to manually implement the data exchange, mostly via an external storage~\cite{klimovic_pocket:_2018,pu_shuffling_2019}, increasing the engineering efforts with additional costs.
Consider as another example the stream where a function needs to process the data accumulated in a time window (Fig.~\ref{fig:data_flow_example} left bottom).
The workflow also fails to express this pattern, as the function is not immediately triggered upon the arrival of data.
Though current serverless offerings allow configuring timers to perform periodic function invocations~\cite{aws_function_timer, azure_function_timer}, it still does not work for the streaming task---there is no knowledge of which data the function should consume, such that developers have to track these data in every time period.
In fact, deploying streaming tasks in current serverless platforms typically needs other cloud services (e.g., AWS Kinesis~\cite{aws_kinesis}) to batch the data for function invocations~\cite{lambda_scenarios,lambda_stream,lambda_stream_example}. 


\begin{figure}[]
    \centering
    \includegraphics[width=0.46\textwidth]{aws_interact}
    \caption{The interaction latency of two Lambda functions under various sizes of data using four approaches. Their performance varies with the data size. In addition, ASF only allows up to 256KB size of intermediate data; Lambda limits the payload size to 6MB; Redis cannot support objects over 512MB. Hence, there is no approach that can always outperform others in any case.}
    \label{fig:aws_interact}
\end{figure}

\PHM{Usability}
As current workflows fail to express a wide range of data sharing patterns, FaaS platforms work around this by providing multiple approaches to function interactions.
For example, functions can exchange intermediate data using a shared storage~\cite{sreekanti_cloudburst_2020,aws_cache,aws_s3,knix,klimovic_pocket:_2018,step_func_large_data}.
They can also be synchronously or asynchronously triggered to process data from nested function call, message queues, and other cloud services~\cite{lambda_invoking}.
However, the presence of many options could complicate function interactions for developers, which in turn affects the usability of FaaS platforms.
In particular, there is no ``best'' approach that can always outperform others in terms of sharing data among functions, forcing developers to figure out by themselves the way to efficiently exchange data for every function pair.



To illustrate this, we compare four approaches to passing data between two Lambda functions: calling a function directly from another (Lambda), letting AWS Step Functions~\cite{aws_step_function} execute the two-function workflow (ASF)~\footnote{We use the Express Workflows in experiments as it delivers higher performance than the Standard Workflows~\cite{step_func_express_workflow}.}, allowing workflow functions to access Redis for fast data sharing (ASF + Redis), and configuring AWS S3~\cite{aws_s3} to invoke the function upon the creation of data (S3)~\cite{lambda_invoke_with_s3}.
Fig.~\ref{fig:aws_interact} shows their latencies under various sizes of data, where no approach can consistently outperform others in any case.
In particular, Lambda achieves the best when transferring small data, but falls short in larger size (e.g., 1MB) and eventually fails on data over 6MB.
While ASF has a more strict limitation on the size, working with fast storage mitigates the problem and delivers better performance until the data reach the maximum object size in Redis.
Using S3 to trigger functions with data transfer is the slowest, but it almost has no limit on data size.
This imposes significant burden on developers to profile the patterns of data exchange and optimize the performance for every pair of interacting functions, especially when there is a large number of functions and various-sized intermediate data in an application.
The problem also lies in other FaaS platforms needing multiple approaches for data sharing, e.g., KNIX~\cite{knix}.

In addition to tuning the performance, developers may require to take into account the interaction cost.
For example, previous works have highlighted the unpleasant trade-off between I/O performance and cost when using different storage to share intermediate data~\cite{pu_shuffling_2019,klimovic_pocket:_2018},
which could further exacerbate the usability problem.

% recommend a storage-based solution~\cite{sreekanti_cloudburst_2020,aws_cache,aws_s3,knix,klimovic_pocket:_2018,step_func_large_data}.
% Functions can write intermediate data to a shared storage, which can be accessed by others when needed.
% While developers can be allowed to explicitly implement various data sharing patterns, this could make function interactions more complex and affect the usability.
% In particular, given the multiple solutions to data sharing, e.g., via workflow or storage, there is no a ``best'' one as their performance varies with the patterns of function invocations and the amount of data to transfer.
% It forces developers to figure out by themselves the way to efficiently transfer data for every function pair.
% directly packing the data into function invocations (Workflow), and using Redis~\cite{aws_cache}---a fast in-memory key-value store---for data exchange (Storage).
% We run two common invocation patterns, parallel and assembling, which respectively perform fanout and fanin with a degree of 2.  
% Fig.~\ref{fig:motivation} shows their latencies with varying data sizes, where no solution can consistently outperform the other in any case.
% It hence can be challenging to optimize the data sharing, especially for workflows having complex patterns of function invocations with a wide range of data sizes.

% In addition, for storage-based data sharing, previous works have highlighted the unpleasant trade-off between I/O performance and cost~\cite{pu_shuffling_2019,klimovic_pocket:_2018}, which exacerbates the usability problem and imposes an undue burden on cloud users.


\PHM{Applicability}
% While the workflow can have various implementations among FaaS platforms~\cite{aws_step_function,azure_durable_function,knix,akkus_sand:_2018,sreekanti_cloudburst_2020}, the performance is far from satisfactory.
Many FaaS platforms could lead to unsatisfactory performance in terms of function interactions~\cite{aws_step_function,azure_durable_function,knix,akkus_sand:_2018,sreekanti_cloudburst_2020}, which significantly limits their applicability.
First, the overhead of function invocations could be too high to enable applications that have stringent latency requirements.
For example, AWS Step Functions can cause a delay of around 20ms when triggering a workflow function without any payload.
It even becomes worse when running more functions in parallel (See more details in~\S\ref{sec:evaluation}), making it ill-suited for latency-sensitive applications~\cite{jia_nightcore_2021}.
Moreover, without efficient support of data sharing, FaaS platforms could be unfit for hosting data-intensive applications~\cite{aws_lambda,knix,jia_nightcore_2021,sreekanti_cloudburst_2020,pu_shuffling_2019,fouladi_encoding_nodate}.
For example, functions can need to exchange large objects through remote storage (Fig.~\ref{fig:aws_interact}), requiring data passing over the network multiple times.
When working on a huge amount of intermediate data (e.g., in analytical workloads), storing and accessing these data for current functions could be a severe performance bottleneck, which we will present in~\S\ref{sec:evaluation}.

The aforementioned three problems significantly undermine the simplicity and appeal of serverless cloud, which motivates the need to systematically enhance the expressiveness and usability of FaaS platforms and improve the performance, i.e., two requirements in~\S\ref{sec:faas_requirement}.
We next present \SysName{}, a new FaaS platform to fulfill these requirements.
In \SysName{} we propose to orchestrate serverless functions following the data---we term this data-centric function orchestration---which can easily enable a variety of new applications  (\S\ref{sec:orchestration}).
We describe \SysName{}'s design for high-performance function interaction in \S\ref{sec:system}.

% We next introduce our design, data-centric orchestration (\S\ref{sec:orchestration}), that fulfills the first requirement. We present our system in~\S\ref{sec:system}, which supports data-centric orchestration with efficient function interactions.

\subsection{FaaS Platform Requirements}
\label{sec:faas_requirement}

% \PHM{Rich Expressiveness and High Usability}
\PHM{Expressive and Ease-of-Use Function Interaction}
As serverless functions are generally stateless without direct communications, FaaS platforms manage their interactions and perform the orchestration at runtime.
A desired FaaS platform should allow developers to easily express the interaction patterns of functions for a wide variety of applications, by that the platform can automatically drive the whole execution without needing developers to manually invoke specific functions and implement data sharing among them.

\PHM{High Performance for Wide Applicability}
A desired FaaS platform also should deliver consistent high performance for any pattern of function interaction, such that it can be widely applied to many applications with different performance requirements.
In particular, the FaaS platform needs to support low-latency function invocations and fast data sharing, regardless of the number of functions to trigger and the amount of data to exchange.
% even in the presence of a large number of functions and a significant amount of intermediate data.


==> contents/orchestration_outdated.tex <==
%!TEX root=../paper.tex
\section{Data-Centric Orchestration}
\label{sec:orchestration}

We first elaborate the key idea of data-centric orchestration.

% In this section, we elaborate the key idea of our approach, followed by its design and programming interface.

\begin{figure}[]
    \centering
    \includegraphics[width=0.46\textwidth]{design}
    \caption{An overview of triggering functions in data-centric orchestration. Source functions write intermediate data to the bucket, which can be configured to automatically trigger target functions using its data when needed.}
    \label{fig:bucket_trigger}
\end{figure}

\subsection{Key Idea}
\label{sec:orch_idea}


% Following the discussion in~\S\ref{sec:deploy_app}, the major problem of workflow-based orchestration is that it only describes the order of function invocations while making data-consuming implicit. In a typically workflow-based serverless platform, each function in the workflow is registered at first. Then, clients specify each function in the workflow and how they are composed. Then results are automatically passed from one function to the fixed target functions during the runtime. 


% From above description, we can find that the workflow-based serverless assumes that the data flow is exactly the same as the function invocation flow. 
% These platforms have no knowledge of the data dependencies between the cloud functions, let alone the amount of data these functions might exchange. 
% % Though the platform got the global view of the whole workflow, it only uses a local view to pass data. 
% Such an assumption restricted its expressiveness severely. For example, when implementing the MapReduce application on a serverless platform, we need to perform data shuffles across stages. The function invocation flow is from the first stage to the second stage. When all the mapper functions finish, it will trigger reduce functions. In a workflow-based serverless platform, because of the above assumption,  it can not decide data flow dynamically based on hash value  during runtime. 
% It fails the shuffle operations due to exploded unnecessary data transfer.

% Thus, if clients of a workflow-based platform want to build applications with complicated data relationships, they should ask for the help of internal/external shared mutable storage, such as s3, Redis, and Anna. In these cases, source functions store intermediate states in shared data storage. Then any other functions can request the data from mutable storage. By using these storage engines, data can flow regardless of function invocation pattern.

% However, the use of shared mutable data storage makes existing serverless platforms far away from ease-to-use (as discussed in 2.3).
% Also, these works ignored that intermediate data is always immutable and short-lived in serverless applications. It is unnecessary to make them durable all the time. Thus, using mutable storage engines brings extra overhead caused by persisting data.
% In this case, the throughput and latency of the mutable storage become the major bottleneck for serverless platforms when dealing with complicated operations like larger shuffles. It limits the applicability of serverless platforms. For example, MapReduce cannot work in practice because shuffle operation does not scale due to object stores latency and IOPS limits.

% As above, workflow-based serverless fails on expressiveness, usability, and applicability due to its assumption that data flow is always following the function invocation flow. Therefore, it motivates us to propose a new design principle: make data-consuming explicit and let data trigger functions, which we define as data-centric. We stress how to share intermediate data when orchestrating functions. In this way, we decouple the data flow and function invocation flow, which will solve the problems described above. 

% Compared to the previous platform, 
%  our platform took advantage of the global view of data consumption. The data flow is not restricted by the function invocation flow anymore. Thus, developers need not implement and optimize the data sharing manually, which will be achieved by the data bucket automatically. 
 %------------
% To illustrate its expressiveness, we take the shuffle operations with m source functions and n target functions as an example again. In our system, we can firstly create a data bucket and divide it with n groups for n reduce functions. We then configure each group to trigger its corresponding reduce function when m objects have received from m source functions. During the runtime, each source function can directly send different data to different data groups by setting different object names. When a group received m objects, it can trigger the reduce function automatically. As described above, shuffle operations can be achieved easily in our system by taking advantage of our data-centric principle.

% Above mechanism enable us to design and implement rich trigger primitives and programming interfaces that make it easy for cients to describe the data flow flexibly and directly.
%------------
%  In sum, the data-centric principle can improve the expressiveness and usability of the serverless platform significantly.

% Furthermore, different with previous works, our data-centric serverless platform do not need shared mutable storage to manage shared state and enable rich expressiveness. Thus, we can take full advantage of the assumption that intermediate data in serverless applications are always immutable and short-lived. 
% It gives us a chance to optimize function interaction using shared memory and local schedulers.  We can let the client choose whether the generated data is durable or not. It will avoid the latency caused by making data persistent when it is unnecessary. During our system design, we keep data sharing in a both efficient and unified manner with different data sizes under different invocation patterns. Our system provides the storage with low-latency, high IOPS based on our evaluation. It will speed up many data-intensive operations and bring better applicability.

We next describe the design of data-centric function orchestration, followed by the programming interface.

% \begin{figure*}[tbp]
%     \includegraphics[width=.98\textwidth]{pri_all}
%     \caption{Usage scenarios of three primitive: \texttt{TimeWindow} for the aggregation in a event stream (left), \texttt{Redundant} for the late binding in ML serving pipeline (center), and \texttt{DynamicGroup} for data shuffle in MapReduce (right).}
%     \label{fig:pri_all}
%     \vspace{-.1in}
% \end{figure*}




\subsection{Design}
\label{sec:orch_design}


\PHM{Overview}
Fig.~\ref{fig:bucket_trigger} gives an overview of triggering functions in data-centric orchestration.
In particular, we design and implement data buckets in our system.

When deploying an application in \SysName{}, it creates one or more data buckets that track intermediate data and serve as function triggers.
 The clients first specify the rule of how the data in a bucket should be consumed. For example, the clients can ask the bucket trigger target functions to consume its accumulated objects in a time window. The bucket can also trigger target functions to consume the objects when specified objects have arrived. We provide 7 common data consumption rules as our trigger primitives, which will be discussed in the next section.

During the runtime, the source function will generate intermediate data. We provide function interface to wrap the data into a named EpheObject. The name can be used as metadata to determine its target function dynamically. Then, source function send these named objects to the specific bucket. Then the bucket checked the data consumption rules set by the clients before.
When the bucket confirms it receives all the objects needed and satisfies the trigger condition, it can trigger the target function and consume these data automatically. 
Above mechanism automatically drives the whole execution.



% As described above, to enable flexible data sharing, we design a variety of primitives for buckets to describe how functions get triggered---we term this \emph{trigger primitive}.
% We next illustrate the primitives implemented in \SysName{}.


% \begin{table}[tb]
%     \centering
%     \footnotesize
%     \caption{The trigger primitives.}
%     \begin{tabular} { | m{6em} | m{21em} | }
%         \hline
%         \textbf{Primitive} & \textbf{Functionality} \\
%         \hline
%         \texttt{UponWrite}  & Trigger the function upon the arrival of any object.  \\
%         \hline
%         \texttt{ByName}  & Trigger the function only when the object name matches a pre-configured value.  \\
%         \hline
%         \texttt{BySet}  & Trigger the function using a set of objects when all is ready.  \\
%         \hline
%         \texttt{ByCount}  & Trigger the function using accumulated objects when the amount reaches a pre-configured number.  \\
%         \hline
%         \texttt{TimeWindow}  & Periodically trigger the function using accumulated objects in a time window.  \\
%         \hline
%         \texttt{Redundant}  & Trigger the function once \emph{k} out of \emph{n} objects ready. \emph{k} and \emph{n} are configurable.  \\
%         \hline
%         \texttt{DynamicGroup}  & Trigger multiple functions, each consuming a unique group of objects. All objects are dynamically divided into groups based on their metadata, e.g., name. \\
%         \hline
%     \end{tabular}
%     \label{tab:primitives}
%     \vspace{-.1in}
% \end{table}

\begin{figure}[]
    \centering
    \includegraphics[width=0.46\textwidth]{figures/cases.png}
    \caption{Usage scenarios of three primitive: \texttt{TimeWindow} for the aggregation in a event stream (left), \texttt{Redundant} for the late binding in ML serving pipeline (center), and \texttt{DynamicGroup} for data shuffle in MapReduce (right).}
    \label{fig:pri_all}
\end{figure}
\PHM{Trigger Primitive}
 As described above, we design and implement data buckets in our system. Functions can send intermediate data as named objects to the data bucket. Then, the data bucket can check the pre-configured data consumption rules. When the rules are satisfied, the data bucket will trigger target functions and consume data. One of the goals of our system is to expose a set of unified and flexible data-sharing interfaces to clients. To achieve this goal, \SysName{} builds on a handful of basic data consumption rules for the data bucket as trigger primitives: direct primitives, conditional primitives, and dynamic primitives.
 
 While the discussion in this section mostly expresses our designed primitives, \SysName{} technically enables developers to extend other trigger rules based on our data-centric model. 
 We stress that data-centric function orchestration provides a general-purpose design paradigm and is not limited to the primitives presented in this section. We make the primitive implementation highly extensible with a common abstraction, allowing the future exploration of more applications.

\emph{Direct Primitives: }
These primitives allow the data bucket to trigger the target function(s) with objects without checking their metadata (e.g. the name), which means we do not make a judgment of the incoming data. So, we refer these primitives as direct consumption. We design three different primitives in this category based on when to trigger these unconditional EpheObjects.
\begin{itemize}
\item UponWrite: Once the data bucket receives one EpheObject, it will trigger the target function(s) with this object. It can enable function chain and broadcast workflow easily.
\item ByCount: Once the data bucket receives a pre-configured number of EpheObjects, it will trigger the target function(s) with all these objects. It will allow the bucket to transfer data in a batch. ~\cite{lambda_stream_example,lambda_stream}
\item TimeWindow: The data bucket periodically triggers the function using accumulated objects it received in a time window. Similar to the ByCount primitive, it also allows the bucket to transfer data in a batch. However, it triggers target function(s) based on time rather than the number of objects. ~\cite{xu_move_2021,chintapalli_benchmarking_2016}
\end{itemize}

\emph{Conditional Primitives: }
Conditional primitives allow the data bucket to check the metadata of the receiving EpheObjects at first, and then decide whether to trigger target function(s). It enables clients to make conditional branches in their data flow graph. So we refer these as conditional primitives. We design three different primitives in this category based on the number of arriving objects.
\begin{itemize}
\item ByName: The data bucket check the name of an incoming  EpheObject. If its name matches the pre-configured one, it will trigger target function(s) and consume the object. It enables conditional function invocations.
\item BySet: Once the data bucket receives all the objects in a pre-configured set, it will trigger target function(s) and consume the set of objects. It is more general than ByName primitive because it can make a decision based on a set of inputs rather than just one.
\item Redundant: Once the data bucket receives k objects in a pre-configured set with n objects, it will trigger target function(s). We can also refer it as BySubset primitive compared to the previous BySet primitive. Redundant primitive supports executing redundant requests and performs late binding. It is meaningful in practice to increase reliability and decrease tail latency.
\end{itemize}

\emph{Dynamical Primitives: }
Above primitives allow data to flow based on pre-configured paths, while dynamical primitive allows dynamically configuring the patterns of data consuming at runtime. We design DynamicGroup for this category.
\begin{itemize}
\item DynamicGroup: In this primitive, the data bucket is divided into groups, and each binds with a target function. At runtime, once the data bucket receives EpheObjcts, it will designate them into different groups based on their metadata. When the trigger condition is satisfied, the data bucket will send different groups to different target functions. For example, in the MapReduce application, map functions can create an Epheobject whose name is its hash value and send the data to different Reduce functions based on this hash value. We will discuss it in detail later.
\end{itemize}



\PHM{Case Study}
The above primitives cover the most common communication primitives in distributed systems, such as direct chain, fan-out, fan-in, and shuffle. Also, it achieves conditional triggering target functions, aggregating data in batch, and configuring data flow dynamically at runtime. These primitives significantly enhance the expressiveness of current serverless platforms. We highlight several usage scenarios in the real world as a case study to illustrate the expressiveness.



\begin{table*}[tb]
    \centering
    \footnotesize
    \caption{The primary API of user library. Users can operate on objects and drive the application execution.}
    
    \begin{tabular}{| m{7em} | m{22em} | m{26em}|}
        \hline
        \textbf{Class} & \textbf{API} & \textbf{Description} \\
        \hline
        \multirow{ 2}{*}{\texttt{EpheObject}} & \texttt{void* \textbf{get\_value}()} & Get pointer to value for this object \\
        \cline{2-3}
        & \texttt{void \textbf{set\_value}(value, size)} & Set value for this object  \\ 
        \hline
        \multirow{ 5}{*}{\texttt{UserLibrary}} & \texttt{EpheObject* \textbf{create\_object}(bucket, key)} & Create object by specifying its bucket and key name \\
        & \texttt{EpheObject* \textbf{create\_object}(function)} & Create object by indicating its target function  \\ 
        & \texttt{EpheObject* \textbf{create\_object}()} & Create object \\ 
        \cline{2-3}
        & \texttt{void \textbf{send\_object}(object, output=false)} & Send object to its bucket, set \texttt{output} flag if it needs to persist \\ 
        \cline{2-3}
        & \texttt{EpheObject* \textbf{get\_object}(bucket, key)} & Get object by specifying its bucket and key name \\ 
        \hline
    \end{tabular}
    \label{tab:api}
    % \vspace{-.1in}
\end{table*}


\emph{Advertisement Stream:}
We take as an example the Yahoo's streaming benchmark~\cite{chintapalli_benchmarking_2016} to illustrate the usage of the \texttt{TimeWindow} primitive.
The benchmark simulates the advertisement analytics pipeline, in that it accepts and filters incoming events of advertisements, check which campaign each relevant event belongs to, and count the events per campaign every second.
Fig.~\ref{fig:pri_all} (left) describes its workflow and how it can be expressed in our design.
Key to porting this application to serverless cloud is ensuring that the last aggregation task is periodically performed on accumulated data.
This can be easily achieved by letting the query function send its results to the bucket, which then automatically triggers the aggregation function with its data once per second.
On the other hand, it would be difficult to implement such task using traditional serverless workflows, which could force developers to track and store these intermediate results (\S\ref{sec:deploy_app}).

\emph{ML Serving Pipeline:}
Serverless computing is well-suited for hosting scalable ML inference services~\cite{zhang_mark:_2019,yu_gillis_icdcs,sreekanti_serverless_serving}.
A ML serving pipeline can have multiple models performing prediction tasks (e.g., classification) in parallel on the same input after prepossessing (e.g., image resizing)~\cite{sreekanti_serverless_serving,crankshaw_inferline_2020}.
ML serving typically needs to meet end-to-end tail latency constraints~\cite{zhang_mark:_2019,crankshaw_inferline_2020,kosaian_parity_2019}, i.e., latency SLOs.
A common approach to reducing the tails is using redundancy~\cite{kosaian_parity_2019}, in that we can issue more requests ($n$) than the need ($k$) in parallel model executions and wait only for the completion of fastest $k$ requests.
This hence mitigates the stragglers and optimizes the tail latency.
In our design such redundant computations can be simply implemented using the \texttt{Redundant} primitive.
Fig.~\ref{fig:pri_all} (center) shows the workflow, where model serving functions directly send the results to a bucket that can trigger the next as long as any $k$ out of $n$ objects arrive.

\emph{MapReduce:}
The fine-grained elasticity of serverless computing makes it promising to host interactive analytical jobs~\cite{muller_lambada_2020,jonas_occupy_2017,pu_shuffling_2019}.
While MapReduce serves as a fundamental and universal programming model in today's data analytics systems~\cite{dean_mapreduce_2008,zaharia_resilient_2011}, it is challenging to directly perform MapReduce-style computations in current FaaS platforms, which requires developers to trigger parallel functions every stage and optimize the data exchange between them~\cite{jonas_occupy_2017,pu_shuffling_2019,klimovic_pocket:_2018} (\S\ref{sec:deploy_app}).
We solve this problem at the level of serverless platform.
Fig.~\ref{fig:pri_all} (right) shows that the \texttt{DynamicGroup} primitive can easily support MapReduce-like operations.
Developers just specify which data groups the intermediate objects belong to when sending them to the bucket.
Once the map functions complete, the bucket automatically triggers a number of reduce functions, each consuming a group of objects.
We will describe how we support an ease-of-programming interface for this application in \S\ref{sec:orch_api}.

\begin{lstfloat}[tb]
\lstset{style=mypython}
\begin{lstlisting}[belowskip=-2.0 \baselineskip, escapechar=|]
app_name = "fan_in"
functions = ['write0', 'write1', 'write2', read]
client.register_app(app_name, functions, [])
client.create_bucket(app_name, 'b_read', NORMAL)
client.add_trigger(app_name, 'b_read', 't_read', 
                  BY_COUNT, 
                  {'function':'read','count':3})
client.call_app(app_name, 
                [(write{i}', [size]) for i in range(3)])
\end{lstlisting}
\caption{Deploy a fan-in application in \SysName{}}
\label{lst:script_client}
\end{lstfloat}

% \begin{figure}[tb]
% \lstset{style=mypython}
% \begin{lstlisting}[belowskip=-2.0 \baselineskip, escapechar=|]
% app_name = "fan_in"
% functions = ['write0', 'write1', 'write2', read]
% client.register_app(app_name, functions, [])
% client.create_bucket(app_name, 'b_read', NORMAL)
% client.add_trigger(app_name, 'b_read', 't_read', 
%                   BY_COUNT, 
%                   {'function':'read','count':3})
% client.call_app(app_name, 
%                 [(write{i}', [size]) for i in range(3)])



% \end{lstlisting}
% \caption{A script to deploy the streaming application using workflow-like interface.}
% \label{fig:many-to-one}
% \end{figure}


\subsection{Programming Interface}
\label{sec:orch_api}




\SysName{} accepts functions written in C++ and allows developers to specify function interactions with a Python client. 
In this section, we start with the function interface and user library, followed by the client and how we simplify the programming.

\begin{lstfloat}[tb]
\lstset{style=interface}
\begin{lstlisting}
int handle(UserLibraryInterface* library, 
           int arg_size, char** arg_values){
    std::string size_str(arg_values[0]);
    int size = stoi(size_str);
    auto ephe_obj = library->create_object(
                    "b_read", 
                    library->gen_unique_key(), 
                    size);
    auto val = static_cast<char *>(
               ephe_obj->get_value());
    memset(val, '1', size);        
    library->send_object(ephe_obj);
    return 0;
}
\end{lstlisting}
\caption{Functions in \SysName{} sending intermediate data}
\label{lst:interface}
\end{lstfloat}


\PHM{Defining Function Interactions}
As described in previous sections, to drive function interactions, \SysName{} allows the user to create data buckets and specify the data consumption rules for the bucket. \SysName{} accepts programs written in Python to specify trigger rules. In particular, the client can be used to configure a number of buckets and assign triggers to them using the primitives described in the previous section, by that the functions can interact with the buckets in creating and sending objects.
After configuring bucket triggers and uploading functions, users issue requests via the client and \SysName{} automatically orchestrate these functions following the order they consume bucket objects.

An simple fan-in example client script is provided in Listing~\ref{lst:script_client}. In line 3, the code specifies the function in the application and registers the application into \SysName{}. Then, the code creates a bucket and adds trigger rules in line 4 and line 5. In this example, we add a trigger to a bucket that triggers the read function after receiving three objects. In line 4, the client invokes the application by calling three write functions. The read function will be orchestrated later automatically.
 
 
\PHM{Function Interface}
As for the function unit, \SysName{} accepts serverless functions written in C++. Listing~\ref{lst:interface} presents the interface for developers to implement their functions. It is similar to the C++ main function, except that it takes the user library as the first argument. The user library provides a set of API functions that allow users to operate on intermediate objects---Table~\ref{tab:api} describes an overview.

% and thus drive the application execution.
The API enables users to create intermediate objects (\texttt{EpheObject}), set their values, and send them to the buckets.
When a bucket decides to trigger the next function, \SysName{} automatically packages the relevant objects as the function augments (Lising~\ref{lst:interface}).
The function can also access other objects via \texttt{get\_object} API if needed.
% Both \texttt{get\_object} and \texttt{send\_object} allow users to interact with a durable storage, specifying whether the object should be fecthed from and persist.
In addition, the \texttt{send\_object} allows users to specify whether the object is the output and should persist after the application completes.

In \SysName{}, users can use our provided UserLibrary to send intermediate data as a named object to the data bucket. Then, the system will pass the data to the target function as its arguments automatically. We provide the same fan-in example to show how to send intermediate data in Listing~\ref{lst:interface}. When sending intermediate data, the write function firstly creates a named EpheObject in a specific bucket. In this example, we use ByCount primitive that doesn't require checking the metadata (name) of the object. Thus, we just give this object a meaningless and unique name. Then, we put the generated intermediate data into the EpheObject. When the data is ready, we send the object to the data bucket.



\begin{figure}[tb]
\lstset{style=mypython}
\begin{lstlisting}[belowskip=-2.0 \baselineskip, escapechar=|]
app_name = 'ad-event-stream'
functions = ['preprocess', 'query', 'count']

dependency_1 = (['preprocess'], ['query'], DIRECT)
dependency_2 = (['query'], ['count'], PERIODIC, 1000)

client.register_app(app_name, functions, \
                    [dependency_1, dependency_2])
\end{lstlisting}
\caption{A script to deploy the streaming application using workflow-like interface.}
\label{fig:script_stream}
\end{figure}
\PHM{Workflow Compatibility}
We also provides a simplified approach to applications that need not to support complex patterns of data consuming by operating on specific objects (e.g., a function chain).
For these applications, \SysName{} allows developers to simply describe the data dependencies among functions using a workflow-like interface.
The interface hides the details of data consuming, where developers only focus on functions and need not to configure triggers and specify buckets in object creation (Table~\ref{tab:api}).
Instead, these can be automatically done by \SysName{} with the knowledge of data dependencies.
This approach hence simplifies the deployment and extends the functionality of current workflow DAG.
We take as an example deploying the advertisement event stream using the script in Fig.~\ref{fig:script_stream}.
There are three functions in the application (line 2), which execute the three tasks in Fig.~\ref{fig:pri_all} (a), respectively.
We can represent their data dependencies as tuples, which specify the source and target functions and indicate how the data should be used. 
In particular, the \texttt{query} function is directly triggered to handle the output of \texttt{preprocess} (line 4), while the \texttt{count} get periodically triggered every 1 second using the accumulated data from the previous \texttt{query} (line 5), which is enabled by the \texttt{TimeWindow} primitive.
The application is simply deployed by registering its functions and dependencies (line 7-8).
% This approach simplifies the deployment of such applications and extends the functionality of workflow DAG.

% We next present our efforts for simplified programming in two scenarios.
% We present two approaches that further simplify the programming for developers in two scenarios, respectively.

\begin{figure}[tb]
\lstset{style=mycpp}
\vspace{-.3in}
\begin{lstlisting}[belowskip=-2.0 \baselineskip, escapechar=|]
void map_function(const char* input, size_t data_size) {
    string input_str{input, data_size};
    vector<string> words;
    split_string(input_str, ' ', words);
    for (auto &w : words) emit(w, 1);
}

void reduce_function(string key, vector<int> &values) {
    int sum = 0;
    for (auto& v : values) sum += v;
    emit(key, sum);
}
\end{lstlisting}
\vspace{.2in}
\caption{WordCount example. Users just need to provide the code snippets of map (line 1-6) and reduce (line 8-12) when using the MapReduce framework atop \SysName{}.}
\label{fig:script_mapreduce}
\end{figure}

\PHM{Case study: }
Our interface can be broadly applied to program many applications, even those having complex data sharing patterns.
For example, it simplifies the orchestration of data processing tasks in a event-driven manner, making it well-suited for running data-flow execution systems~\cite{dean_mapreduce_2008,zaharia_resilient_2011}.
To illustrate this, we build a MapReduce framework atop \SysName{}, named \SysName{}-MR.
The framework is backed by the \texttt{DynamicGroup} primitive (Fig.~\ref{fig:pri_all}(c)). 
% and simply implemented using current interface (Table~\ref{tab:api}).
% The framework can simply implement MapReduce operation by leveraging the \texttt{DynamicGroup} primitive (Fig.~\ref{fig:pri_all} and  the current interface (Table~\ref{tab:api}).
Fig.~\ref{fig:script_mapreduce} gives an example of running the WordCount atop \SysName{}-MR, which works as follows.
The framework first configures bucket triggers and accepts the code snippets of map and reduce from users, which are packaged into two \SysName{}'s functions (Listing~\ref{lst:interface}), respectively.
The actual map functions execute the user-provided code and then automatically send out intermediate objects while indicating their targets in the names.
Reduce functions thus get triggered to aggregate these objects and output the final results.
In this case, framework users can simply focus on the logic of the MapReduce program.
In addition, \SysName{}-MR only needs 380 lines of C++ function wrappers and 120 lines of Python interface.
Given that PyWren~\cite{jonas_occupy_2017} is programmed in about 6K lines of Python for executing large-scale map operations on Lambda, \SysName{} significantly reduces the engineering efforts for framework developers.
% when porting frameworks to the serverless cloud.

